On Slowly-varying Non-stationary Bandits

We consider minimisation of dynamic regret in non-stationary bandits with a slowly varying property. Namely, we assume that arms' rewards are stochastic and independent over time, but that the absolute difference between the expected rewards of any arm at any two consecutive time-steps is at most a drift limit $\delta > 0$. For this setting that has not received enough attention in the past, we give a new algorithm which extends naturally the well-known Successive Elimination algorithm to the non-stationary bandit setting. We establish the first instance-dependent regret upper bound for slowly varying non-stationary bandits. The analysis in turn relies on a novel characterization of the instance as a detectable gap profile that depends on the expected arm reward differences. We also provide the first minimax regret lower bound for this problem, enabling us to show that our algorithm is essentially minimax optimal. Also, this lower bound we obtain matches that of the more general total variation-budgeted bandits problem, establishing that the seemingly easier former problem is at least as hard as the more general latter problem in the minimax sense. We complement our theoretical results with experimental illustrations.

==> arXiv version/abstract.tex <==
\begin{abstract}

We consider minimisation of dynamic regret in non-stationary bandits
with a slowly varying property. 
Namely, we assume that arms' rewards are stochastic and independent over time,
but that the absolute difference between the expected rewards
of any arm at any two consecutive time-steps is at most a drift limit $\delta > 0$.
For this setting that has not received enough attention in the past, 
we give a new algorithm which extends naturally the well-known Successive
Elimination 
% \cite{even2002pac} 
algorithm to the non-stationary bandit setting.
We establish the first instance-dependent regret upper bound
for slowly varying non-stationary bandits. 
The analysis in turn relies on a novel characterization of the instance 
as a {\em detectable gap} profile that depends on the expected arm reward differences.
We also provide the first minimax regret lower bound for this problem,
enabling us to show that our algorithm is essentially minimax optimal.
Also, this lower bound we obtain matches that of the more
general total variation-budgeted bandits problem, 
establishing that the seemingly easier former problem is at least as hard as the
more general latter problem in the minimax sense. 
We complement our theoretical results with experimental illustrations.

\end{abstract}

==> arXiv version/algorithm.tex <==
\section{ALGORITHM DESCRIPTION}
\label{sec:algorithm}

Successive Elimination (SE) is a well-known algorithmic recipe for solving stationary stochastic bandits, built upon the Explore-Then-Commit (ETC) paradigm 
(see \cite{slivkins2019introduction} for a text-book treatment of SE and ETC)
In its classical form, SE adaptively pulls both arms alternately until it distinguishes the optimal arm from the sub-optimal (in terms of reward means) with a high probability. Then, it drops the inferior arm and indefinitely plays the superior arm.
% It is known that Successive Elimination enjoys a minimax optimal regret upper bound.
Our algorithm, $\AlgGE$ (Algorithm \ref{alg:gauge-enjoy}), is a graceful adaptation of the Successive Elimination paradigm to the non-stationary bandits setup.
It pulls arms alternately until it can assertively distinguish the two arms in a `local average' sense, 
and then plays only the optimal arm for a period of time until the sub-optimal arm, due to the non-stationarity, can become the optimal arm.

Specifically, the $\AlgGE$ algorithm runs in a series of episodes.
Every episode begins with an \emph{active phase}, where $\AlgGE$ pulls the two arms alternately (in a round-robin fashion). 
At the end of every time-step, it performs a statistical test (Line \ref{line:stat-test} ) to detect a \emph{clear gap} (in reward means) between the two arms.
If the test succeeds, the active phase ends and the observed sub-optimal arm is possibly
\emph{snoozed} for a certain period of inactivity 
(Lines \ref{line:check-snooze-condition}-\ref{line:snooze}),
termed as the \emph{passive phase}.
During this passive phase, $\AlgGE$ plays only the observed optimal arm.
At the end of this passive phase, the observed sub-optimal arm \emph{respawns} to become active, and the next episode begins.

We introduce some notations to describe the statistical test and for the analysis in the remainder of the paper.

Let $e$ be the total number of episodes (indexed as $1,2,\dots,e$) in a run of $\AlgGE$.
For every episode $i \in [e]$, let $t_i$ denote the time after which the active phase of episode $i$ begins. Note that $t_{i+1}$ corresponds to the time at which episode $i$ ends. We also always have $t_1 = 0$ and $t_{e+1} = T$, the end time of the final episode.
Let $g_i$ denote the time at which the statistical test on line \ref{line:stat-test} of the algorithm passes, 
and write $\tau_i := g_i - t_i$ to denote the duration of the active phase of episode $i$. %

Write $\muhat_{a,t}(w)$ to denote the empirical reward mean (or simply empirical mean) of arm $a$
at time $t$ measured/calculated from it's last $w$ pulls, i.e., the most recent $w$ pulls until time $t$.
Note that the true reward means $\mu_{a,t'}$ for different time-steps $t'$
corresponding to these last $w$ pulls 
% (in period $[t_i, t]$) 
need not be the same.

\begin{definition}[$\lambTil$-betterness]
\label{def:lambda-better}
Let $\lambTil > 0$. At time $t$, in the active phase of episode $i$,
 % \in [0,1]$,
arm $a$ is said to be $\lambTil$-better than arm $b$ 
(written as $a \lambTilGreat b$) if, 
for a window sample count $w := \ceil{\frac{c_1 \log T}{\lambTil^2}} \leq \frac{t-t_i}{2}$, 
we have $ LCB_{a,t}(w) > UCB_{b,t}(w) + 2 r(w) - \delta$,
and the inequality holds for no other $\lambTil' < \lambTil$.
\end{definition}

In the above definition, write
$LCB_{a,t}(w) := \muhat_{a,t}(w) - r(w)$  
($UCB_{b,t}(w) := \muhat_{b,t}(w) + r(w)$)
to denote the lower (upper) confidence bound of arm $a$'s ($b$'s) recent reward mean,
and $r(w) := \sqrt{\frac{2\log T}{w}}$ 
is the accuracy radius with $w$ samples.
The constraint $w \leq \frac{t-t_i}{2}$ ensures that
the samples used in the statistical test (or comparison expression in the definition) are all from the (current) episode $i$.

In the statistical test (Line \ref{line:stat-test}) at a time $t$, 
$\AlgGE$ evaluates if some arm is $\lambTil$-better than the other (as in definition \ref{def:lambda-better})

Essentially, it compares the empirical means of the two arms
measured over a window of samples ending at $t$, the $\muhat_{a,t}(w)$s. 
% to detect an empirical detectable gap of any possible $\lambTil \in [0,1]$.

The size of the window, $w$, in which the empirical means are calculated is dynamically chosen based on the empirical detectable gap, $\lambTil$, istelf that is being tested for.
If the test passes, then $\AlgGE$ computes 
a sub-optimality buffer period of duration $\text{buf}=\frac{2}{\delta} \sqrt{\frac{\log T}{\tau_i}}$ (Line \ref{line:compute-buffer}), 
% in which sub-optimal arm can never become optimal... ??
that began no earlier than the start of the current episode $t_i$.
By time $t$, if the buffer period has not fully elapsed, 
we snooze the sub-optimal arm for a passive phase that runs until the end of the buffer period.
% We shall show (in Lemma \ref{}) that no regret is incurred during such a passive phase.

\begin{remark}
\label{rem:computation-in-stat-test}
    The statistical test (Line \ref{line:stat-test}) describes the identification of a $\lambTil$-better arm 
    as an optimization problem over the continuous domain $\lambTil \in [0,1]$. 
    However, with the integrality constraint of the sample window size $w$ corresponding to a $\lambTil \in [0,1]$,
    we have $w \in D \subseteq \{1,2, \dots, t\}$ belongs to a finite countable domain of size not more than $t$.
    Thus, the identification of a $\lambTil$-better arm becomes a discrete optimization problem,
    and indeed, the statistical test is deterministic and tractable. 
\end{remark}

\begin{algorithm}[h]
\small
\caption{$\AlgGE$: Plays the non-stationary slowly-varying bandit problem instance}
\label{alg:gauge-enjoy}
{\bf Input:} Time horizon $T$, a set of two arms $\Arms=\{1,2\}$ with sample access, the drift limit $\delta$.\\
{\bf Output:} Play an arm for every time-step. 
\begin{algorithmic}[1]
    \State Initialize set of active arms $A = \Arms$,
    set of snoozed arms $S = \emptyset$.
    \State Initialize episode index $i \leftarrow 1$, $\tau_1 = 0$.

    \For{$t = 1,2,\dots,T$}
        \State $x \leftarrow$ Least recently pulled arm in $A$.
        \Comment{Play active arms in round-robin fashion}
        \State Pull arm $x$ and observe reward $\muhat_{x,t}$.
        \label{line:pull}
        \If{$\exists$ arms $a,b \in A$, $\exists \lambTil \in [0,1]$ s.t. $a \lambTilGreat b$}
        \label{line:stat-test}
        \Comment{As in Definition \ref{def:lambda-better}}
            \State Statistical test success time, $g_i = t$
            \State Active phase duration, $\tau_i = g_i - t_i$.
            \State Sub-optimality buffer, $\text{buf} = \dfrac{2}{\delta} \sqrt{\dfrac{\log T}{\tau_i}}$
            \label{line:compute-buffer}
            \If{$\text{buf} > \tau_i$}
            \label{line:check-snooze-condition}
                \State $A \leftarrow A \setminus \{b\}$
                \State $S \leftarrow S \cup \{(b, t_i + \text{buf})\}$
                \label{line:snooze}
                \Comment{Snooze arm}
            \Else
                \State $i \leftarrow i+1, t_i \leftarrow t$
                \Comment{End episode without passive period}
            \EndIf
        \EndIf
 
        \If{$\exists (x,s) \in S: s \geq t$}
            \State $S \leftarrow S \setminus \{(x,s)\}, 
                     A \leftarrow A \cup \{x\}$
            \Comment{Respawn arm}
            \State $i \leftarrow i+1, t_i \leftarrow t$
            \Comment{End episode for passive period elapses}
        \EndIf
    \EndFor
\end{algorithmic}
\end{algorithm}

Optionally, we refer the reader to appendix \ref{appn-subsec:missing-figures} (figures \ref{fig:alg-trajectory-1} and \ref{fig:alg-trajectory-2}) for a graphical example of an algorithmic trajectory
that illustrates the active phases, statistical tests, and snooze periods.


==> arXiv version/conclusion.tex <==
\section{CONCLUSION}

%For the slowly-varying bandits, we provided an algorithm $\AlgGE$ that is a graceful extension of the Successive Elimination design
%to the non-stationary setup. 
%We established the first  instance-dependent regret bound in the drifting bandits regime.
%Towards that, we developed a novel characterization of the problem instance that we term detectable gaps.
%Finally, we proved a novel lower bound for the slowly-varying bandits problem, that,
%not only showed that our algorithm is minimax optimal, but also that the slowly-varying bandits problem is at least
%as hard as the more general total variation-budgeted bandits setting.
% Come on, how many times have we said this in this paper?

Our characterization of the detectable gap profile enabled an instance-dependent characterization of the regret in the drifting setting. We believe that the detectable gap profile 
is a fundamental property of non-stationary bandit settings that may hold the key to more refined performance analysis, beyond merely the slowly-varying setting considered here. On that note, one interesting direction to pursue would be to characterize instant-dependent regret bounds
in the more general total variation-budgeted setting.



==> arXiv version/experiments.tex <==
\section{NUMERICAL RESULTS}
\label{sec:experiments}
 
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[b]{0.46\textwidth}
            \centering
            \includegraphics[width=\linewidth]{Resources/Instance17_Regret.png}
            \caption{}
            \label{fig:regret-low-delt-well-sep}
    \end{subfigure}%
    \begin{subfigure}[b]{0.4\textwidth}
            \centering
			\includegraphics[width=\linewidth]{Resources/Instance15_Regret.png}
            \caption{}
            \label{fig:regret-high-delt-oscillating-arms}
    \end{subfigure}
    \caption{Comparison of average regret among the 4 algorithms. The translucent regions (of the same colour) around the curves mark 1 standard deviation over 10 runs. 
    }
\end{figure*}

\begin{figure*}[!h]
    \centering
    \begin{subfigure}[b]{0.47\textwidth}
            \centering
		    \includegraphics[width=\linewidth]{Resources/delta_comp_reg_5.png}
            \caption{}
            \label{fig:regret-snoozeit-multi-delta-1}
    \end{subfigure}%
    \begin{subfigure}[b]{0.44\textwidth}
            \centering
			\includegraphics[width=\linewidth]{Resources/delta_com_reg_4.png}
            \caption{}
            \label{fig:regret-snoozeit-multi-delta-2}
    \end{subfigure}
    \caption{Comparison of average regret incured by $\AlgGE$. The translucent regions (of the same colour) around the curves mark 1 standard deviation over 10 runs. }
\end{figure*}


We numerically evaluate the performance of $\AlgGE$\footnote{
	As noted in Remark \ref{rem:empirical-tweaks}, we slightly modify our algorithm 
	(as in appendix \ref{appn-subsec:modified-algo}) to possibly realise its full potential.} on synthetic problem instances. We also implement algorithms from the literature and conduct a comparative study with different problem instances.
In particular, we consider the following algorithms; 
(1) $\rexp$ \citep{besbes2014stochastic}, that divides the time into blocks upfront and repeatedly runs the Exp3 algorithm 
% (introduced in ) 
from scratch in each block,
(2) $\swucb$ \citep{wei2018abruptly}, a soft exploration algorithm based on the arms' reward means' upper confidence bounds that are computed over a sliding window that enlarges with time.
(3) $\exps$ \citep{besbes2019optimal}, a `smoother' variant of Exp3 algorithm.
%  Not necessary to further cite Freund & Schapier '97 for the Exp3 algorithm.
We note that $\rexp$ and $\exps$ are originally proposed for the more general total variation-budgeted setting.
Also, all these algorithms have knowledge of the drift limit $\delta$ (or the appropriate drift parameter) in advance.

We consider a time horizon of $T\simeq 160,000$, 
and report results averaged from 10 runs. 
The rewards are drawn from a Gaussian distribution with the specified mean, and a variance of \nicefrac{1}{4}.
\footnote{Indeed, the choice of a Gaussian draw with \nicefrac{1}{4} variance fits in with our theoretical analysis, specifically, the Hoeffding's inequality usage in Claim \ref{clm:good-event-prob}}.
% Bern has very low variance as p->0/1 stuff is not necessary.

First, we run all the algorithms on a problem instance 
with a low value of local change   $\delta=\nicefrac{1}{(10 c_9 \log T)} \simeq 0.000021$  where the arms are well-separated (refer to  fig. \ref{fig:instance-low-delt-well-sep} in appendix \ref{appn-subsec:missing-figures}). The identity of the optimal arm remains unchanged throughout.
We observe (fig. \ref{fig:regret-low-delt-well-sep}) that $\rexp$ and $\exps$ perform poorer compared to
$\swucb$ and $\AlgGE$. 
While $\AlgGE$ and $\swucb$ are very adaptive in their behaviour to the observed empirical reward means,
we see that $\rexp$ predetermines the sizes of blocks (tailored to the drift parameter),
and $\exps$, after tuning the weights, additionally boosts up the weights of the arms equally without taking into account the observed empirical gaps.
% thereby, the weight of the perennially sub-optimal arm fails to significantly and quickly decrease, resulting in it being pulled more often.
%Note, however, that $\exps$ was designed to handle more general problem instances and expectedly does not exploit the empirical gaps as much as one can in the slowly-varying bandits setup. 

Second, we run all 4 algorithms on a problem instance 
 with a relatively larger value of local change $\delta=\nicefrac{1}{( c_9  \log T)} \simeq 0.00021$, where both arms have short alternating stretches of stationarity and drifts, with the identity of the optimal arm toggling with every drift (fig. \ref{fig:instance-high-delt-oscillating-arms} in appendix \ref{appn-subsec:missing-figures}).
Interestingly, we observe (fig. 
\ref{fig:regret-high-delt-oscillating-arms}) that $\swucb$ performs poorer compared to $\AlgGE$. 
We hypothesise that $\AlgGE$ makes better use of short frequent stretches of stationarity; 
% by the nature of its statistical test;
% however, $\swucb$ owing to its short sliding window size (due to larger $\delta$) explores more than it would otherwise;
however, with the arms oscillating as we have here, when the sliding window encompasses the optimal stretches (and the drifts) of both arms,
$\swucb$ does not take into account the recency of the samples within the sliding window. 
% thereby not learning much useful details about the state of the instance.
$\AlgGE$, on the other hand, operates with dynamically-sized windows based on the observed detectable gaps that always capture the most suitably sized number of recent samples.

Third, we evaluate the performance of our algorithm on different instances.
In particular, we consider 4 instances with similar structure that differ only by the drift limit $\delta$ imposed, and have common periods of stationarity and drift
(refer fig. \ref{fig:instance-snoozeit-multi-delta-1} in appendix \ref{appn-subsec:missing-figures}).
We observe (fig. \ref{fig:regret-snoozeit-multi-delta-1}) that the average regret does not correlate with an increase in drift limit $\delta$. 
The well separated nature of the arms in instances with a higher $\delta$ improves performance (specifically, increased detected (empirical) gaps lengthen the snooze periods),
and potentially offsets the higher regret causable due to more frequent episodes (specifically, larger $\delta$ values shorten the snooze periods).

Finally, we consider another set of 4 structurally similar instances with different $\delta$, where arms have equal total cumulative drift and almost common periods of stationarity and drift (refer fig. \ref{fig:instance-snoozeit-multi-delta-2} in appendix \ref{appn-subsec:missing-figures}). 
With the same maximum gaps among instances, the regret increases with drift limit $\delta$ (fig. \ref{fig:regret-snoozeit-multi-delta-2}), which is in line with what our theory lays down.



==> arXiv version/introduction.tex <==
\section{INTRODUCTION}

Reinforcement learning, and specifically bandit optimization, in dynamically changing environments has remained an active topic of study in machine learning. A variety of non-stationary bandit settings have been studied incorporating a range of structural assumptions. At one end are classical stochastic models such as restless bandits \citep{whittle1988restless}, where the state of the arms governs the bandit problem at any instant, but the transitions between these problems (states) follow probabilistic dynamics. At the other extreme are settings with non-stochastic and arbitrarily changing rewards such as prediction with expert advice (and the EXP3 algorithm)\citep{cesa2006prediction, auer2002nonstochastic}.
% , \cite{auer2002nonstochastic}. 
In between these extremes lie settings of changing environments where the adversary (environment) is assumed to be limited in its ability to change the rewards, i.e., a structural constraint is put on the amount of change in the rewards across time. These include the abrupt change (or switching experts) model \citep{garivier2011upper}, where at most $k$ arbitrary changes to the reward distributions are allowed in the entire time horizon, and the variation-budgeted (drifting) change model \citep{besbes2014stochastic}, in which the total magnitude of changes (of rewards) across successive time steps is constrained to be within an overall budget.

In this paper, we focus on slowly-varying bandits -- a different and arguably commonly encountered, yet less studied, model of non-stationary bandits. 
In this setting, the arms are allowed to change arbitrarily over time as long as the amount of change in their mean rewards between two successive time steps is bounded uniformly across the horizon.
Many real-world settings naturally involve observables whose distributions are `smooth' over time, in the sense that their instantaneous rate of change is not too large, e.g., slowly drifting distributions in natural language tasks \citep{lu2020countering}, data from physical transducers (position, velocity, power, temperature, chemical concentration), and slowly fading wireless channels \citep{tse2005fundamentals}. Though the slowly-varying bandit setting is subsumed by the total variation-budgeted model with an appropriate budget, the hope is that the local smoothness of the rewards with time can be exploited by the learner to perform better. We make the following contributions in this regard. 

\begin{enumerate}
	\item We give a new algorithm for slowly-varying two-armed bandits. The algorithm is based on the principle of adaptive exploration followed by commitment in phases -- a strategy that is known to be optimal for stationary stochastic bandits -- but where the commitment phase is adjusted depending on the smoothness constraint on the rewards. The design of the algorithm also involves the estimation of a novel property of the bandit instance called the detectable gap profile, which essentially characterises the gap between the local averaged means of the arms that can be reliably detected, across time.
	
	\item We derive a regret bound for this algorithm in terms of the detectable gap profile of the bandit instance (Theorem \ref{thm:inst-dep-reg}). The bound, to our knowledge, is the first instance-dependent regret guarantee for any algorithm for drifting stochastic bandits. Moreover, the worst case regret bound for a horizon $T$, over all instances for a given constraint $\delta$ on instantaneous reward change, is shown to be $O(T \delta^{\nicefrac{1}{3}})$ (Theorem \ref{thm:minimax-bound}).
	
	\item We complement this worst case regret upper bound with a matching fundamental lower bound (Theorem \ref{thm:lower-bound}) -- the first of its kind for slowly-varying bandits -- that shows that our algorithm is order-wise minimax-optimal. Interestingly, the minimax regret rate happens to be the same as that of the total variation-budgeted (with equivalent budget $\delta T$) setting, establishing that the more constrained slowly-varying setting is at least as hard (in a worst case sense) as the more general total variation-budgeted setting. 
	
	\item We numerically evaluate the performance of our new algorithm and existing approaches, showing that there are situations in which it is able to outperform the other approaches. 
\end{enumerate}

\input{related-work}











==> arXiv version/nice_packages.tex <==
%% Language and font encodings
% \usepackage[english]{babel}
% \usepackage[utf8x]{inputenc}
% \usepackage[T1]{fontenc}

%% Sets page size and margins
% \usepackage[top=3cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}

% Siddharth's Arxiv format
\usepackage[margin=0.8in]{geometry}
\renewcommand{\familydefault}{ppl}

% \usepackage{authblk}

\usepackage{amsfonts, amsmath, amssymb, amsthm}
% \usepackage{amsart} % Has the substack command.
\usepackage{mathtools} % Has the DeclarePairedDelimeter macro and maybe more.

% \usepackage{mathalpha}
\usepackage{bm}
\usepackage{verbatim}
\usepackage{euscript}
\usepackage{graphicx}
\usepackage{paralist}
\usepackage{cancel} % to strike-out terms in an equation.

% Package for indicator random variable?! %
\usepackage{bbm}

\usepackage{nicefrac}

% Restatable claim/lemma/theorems
\usepackage{thmtools,thm-restate}


% MATHS NOTATIONS
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
% \DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
% \DeclarePairedDelimiter\ceil{\left \lceil}{\right \rceil}
% \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand{\abs}[1]{\left \lvert #1 \right \rvert}
% \newcommand{\norm}[1]{\left \lfloor #1 \right \rfloor}
\newcommand{\maxtwo}[2]{ \max \left \{ #1, #2 \right \} }

\newcommand{\cardinality}[1]{ \left\lvert #1 \right\rvert }
% PROBABILITY NOTATIONS
\newcommand{\ceil}[1]{\left \lceil #1 \right \rceil}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor}

\newcommand{\prob}[1]{\mathbb{P} \left\{ #1 \right\}}
\newcommand{\probover}[2]{\underset{#1}{\mathbb{P}} \left[ #2 \right]}
\newcommand{\probunder}[2]{\mathbb{P}_{#1} \left\{ #2 \right\}}
\newcommand{\probdistunder}[1]{\mathbb{P}_{#1}}

\newcommand{\expectation}[1]{\mathbb{E} \left[ #1 \right]}
\newcommand{\expectationover}[2]{\underset{#1}{\mathbb{E}} \left[ #2 \right]}
\newcommand{\expund}[2]{\mathbb{E}_{#1} \left[ #2 \right]}
\newcommand{\indicator}[1]{\mathbbm{1} \left\{ #1 \right\}}
\newcommand{\inprod}[2]{\langle #1 , #2 \rangle}

% ORDER NOTATIONS
\newcommand{\bigO}[1]{O \left( #1 \right)}
\newcommand{\bigTheta}[1]{\Theta \left( #1 \right)}
\newcommand{\bigOmega}[1]{\Omega \left( #1 \right)}

\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{soul}
\usepackage{float}

\usepackage{xspace}
\usepackage{wrapfig}

%\usepackage{caption} % Custom captions for tables etc.

\usepackage[usenames,dvipsnames]{color}
\usepackage{xcolor}

\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true, allcolors=black]{hyperref}

% Specify bibliography package
\usepackage{natbib}

% Packages for algorithms
\usepackage{algorithmicx, algpseudocode}
\usepackage[ruled]{algorithm}

% For strike through of text
\usepackage[normalem]{ulem}

% CUSTOM CREATED COMMANDS

% Command for numbering equations within align* env 
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

% \renewcommand\qedsymbol{$\blacksquare$}



% GREEK STYLE OF RESEARCH
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{observation}{Observation}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{remark}{Remark}

\newtheorem{claim}[lemma]{Claim}
\newtheorem{fact}[lemma]{Fact}
\newtheorem{conjecture}[lemma]{Conjecture}
\newenvironment{assumption}{\noindent{\bf Assumption}\hspace*{1em}\begin{em}}{\end{em}\medskip}
\newenvironment{remark-nolabel}{\noindent{\bf Remark}\hspace*{1em}}{\bigskip}

\newcommand{\IR}{\mathbb{R}}
\newcommand{\muhat}{\widehat{\mu}}

% The colours of hyper-links 
\hypersetup{
  colorlinks   = true, %Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = blue, %Colour of internal links
  citecolor   = blue %Colour of citations, could be ``red''
}

% Artifical comment tag. Takes an argument and does nothing.
% \def\ignore[1]{}
\long\def\comment#1{}
\long\def\thought#1{\textcolor{red}{#1}}
\newcommand{\slfrac}[2]{\left.#1\middle/#2\right.}

% \newcommand{\b}[1]{\textbf{#1}}
\newcommand{\bi}[1]{\textbf{\textit{#1}}}
\newcommand{\biu}[1]{\underline{\textbf{\textit{#1}}}}
\newcommand{\iu}[1]{\underline{\textit{#1}}}
% \newcommand{\i}[1]{\textit{#1}}
% \newcommand{\u}[1]{\underline{#1}}
\newcommand{\bu}[1]{\underline{\textbf{#1}}}


==> arXiv version/preliminaries.tex <==
\section{SETTING AND PRELIMINARIES}

We consider bandits with arm set $\Arms = \{1,2\}$
\footnote{We restrict to two arms because we would like to focus on understanding the dependence of regret on the non-stationarity over \emph{time} as opposed to over the arm space. 
This is also the line of investigation adopted in other works on non-stationary bandits for similar reasons 
(\cite{auer2018adaptively}, \cite{karnin2016multi})} and a time horizon of $T$.
% \footnote{We shall interchangeably use the term 'time horizon' to mean the actual series of time-steps $[1,2,\dots,T]$ and the total number of time-steps $T$.}
At time $t \in [T]:=\{1,2,\dots,T \}$, when arm $a \in \Arms$ is pulled by a bandit algorithm, depending on only past history, a stochastic reward is drawn from a Bernoulli
\footnote{In general, our theoretical analysis and results hold for any sub-gaussian reward distributions with a suitably bounded variance.} distribution with expected value $\mu_{a,t} \in [0,1]$ is obtained.
% the expected reward mean of arm $a$ at time $t$.
We denote by $\mu_t := (\mu_{1,t}, \mu_{2,t})$ the expected reward tuple at time $t \in [T]$, 
and denote by $\mu^*_t = \max_{a \in \Arms} \mu_{a,t}$ the optimal arm (in terms of expected reward) at time $t$.
Write $\mu := (\mu_1, \mu_2, \dots, \mu_T)$ be the expected reward profile of the bandit instance.

A bandit instance $\mu$ is defined to be  \emph{slowly-varying} with \emph{drift limit} $\delta > 0$ (denoted as $\mu \in S_\delta$) if the expected reward profile satisfies
% The above verbose 'drift' stuff can be moved to Introduction when we motivate the setting. A more formal statement can be used here. RAMA
\begin{align*}
    \forall a \in \Arms, t \in [T-1], \abs{\mu_{a,t}-\mu_{a,t+1}} \leq \delta. \numberthis \label{eqn:drift-limit}
\end{align*}
In other words, for an arm $a \in \{1, 2\}$ at a time step $t$, the expected reward $\mu_{a,t}$ can drift in value to some $\mu_{a,t+1}$ (the next time-step) by at most $\delta$.

% Equivalently (actually more powerfull, but unjustifiable to possess knowledge of that exact $\delta$),
% we define the drift limit as 
% $\delta = \max_{t=1}^{T-1} |\mu_{a,t} - \mu_{a,t+1}|$.

%A slowly-varying bandit problem instance is fully characterized by the tuple $\left(\mu, \delta \right)$.
% Here, we (justifiably?) assume that $\delta$ is known upfront (to the algorithms).

%Next, we define the regret expression that we consider in our setting.

\begin{definition}[Regret]
    For a bandit instance $\mu$, the (expected) regret  
    incurred by an algorithm $\Alg$ is
    \begin{equation*}
        R(\Alg) = \sum_{t=1}^T \mu^*_t - \expectation{\mu_{\Alg(t), t}},
    \end{equation*}
    where $\mu^*_t = \max_{a \in \Arms} \mu_{a,t}$ is the mean reward of the optimal arm at time $t$,
    and $\Alg(t) \in \Arms$ is the arm pulled by $\Alg$ at time $t \in [T]$.
\end{definition}

Note that this is the \emph{dynamic regret}, where 
the performance benchmark at each time-step is the expected reward of the optimal arm at that time-step ($\mu^*_t$).
This is a stronger (i.e., harsher) notion of regret compared to the classical notion of \emph{static regret}, where
the benchmark at all time-steps is the expected reward of the best single arm across the entire horizon in hindsight.

The goal is to learn to play arms to achieve low (dynamic) regret
for any problem instance $\mu \in  S_\delta$.
 
We assume that the algorithm has access to the drift limit $\delta$ (or a suitable upper bound on it). 
This is reasonable as in practice
there is often domain specific information available in advance about the drift of the 
quantity in consideration.
%with the knowledge of the drift limit $\delta$ and time horizon $T$ given upfront.

% We next present a derived characterization (from instance $\mu$) of the problem for ease of analysis.
We now introduce a novel characterization of a non-stationary bandit instance, and highlight its significance to the algorithm design and analysis to follow later.

% We define a sub-optimality/gap arc/curve/function that tracks the difference/gap between the (or a) sub-optimal arm and the optimal arm at every time-step.

\paragraph{Gaps and Detectable Gap Profile.}
%  THIS PARAGRAPH SHOULD IDEALLY HAVE NOTHING TO DO WITH SLOWLY-VARYING ASPECT.

\begin{figure*}[!h]
    \centering
    \makebox[\textwidth][c]{
    \includegraphics[width=1.1\linewidth]{Resources/Lambda_Description_backup.png}
    }
    \caption{Depiction of the arms' true reward means, the gap profile, and the detectable gap profile of one problem instance illustrated at 4 zoom levels. The box in each image is the region zoomed in for the next image (to its right).
    First, the detectable gaps ($\lambda$) reasonably positively correlates with the gaps ($\Delta$), and initially (in general, whenever there is not a sufficient window size to detect a gap), for a short span, it takes the form $\sqrt{\frac{c_0 \log T}{t}}$.
    Second, $\lambda$ roughly trails $\Delta$ as it depends on a recent window of $\Delta$ at every time-step.
    Third, $\lambda$ is `smoother' compared to $\Delta$, as by design, its values are averaged over a window of samples.
    Fourth, although $\lambda$ is described as a continuous optimization problem over $[0,1]$, 
    % by the constraints of integrality of window size $w$, 
    it actually transforms into a discrete optimization problem over different integral window sizes $w$. Thus, $\lambda$ has a `piece-wise constant' appearance.}
    \label{fig:lambda-description}
\end{figure*}

In the {\em stationary} stochastic (two-armed) bandit problem, the suboptimality \emph{gap} $\Delta := \abs{\mu_1 - \mu_2}$ essentially characterises the attainable regret rate\footnote{assuming bounded/sub-gaussian rewards}. 
With {\em non-stationary} reward distributions, the notion of a (time-invariant) gap must be generalised to a {\em gap profile}
$\Delta := (\Delta_t)_t$ where $\Delta_t := \abs{\mu_{1,t} - \mu_{2,t}}$ is the difference 
at time $t$ between the expected rewards of the two arms, $\mu_{1,t}$ and $\mu_{2,t}$.

% Note that because of the step-wise drift constraint of the arms, 
% the gap profile/list is constrained by 
% $|\Delta_t - \Delta_{t+1}| \leq 2\delta$ 
% for all time-steps $t=[1,T-1]$.

%In a non-stationary setting, however, the instantaneous gap $\Delta_t$ %
%%does not sufficiently capture the state of the problem instance at a particular time. 
%does not convey any useful information about the nature of non-stationarity at that time. %
%%and thus the nature of the problem instance in its temporal neighbourhood.
%% This is a crucial detail that impacts

We now introduce the notion of a {\em detectable gap profile} $\lambda := (\lambda_t)_t$, which intuitively helps to characterise how hard it is to reliably estimate which arm is optimal and by how much at any time $t$. This is a derived quantity expressed in terms of the gap profile taken over a local window of time leading up to $t$. %
%needs samples over a sustained time period.
%So, it becomes necessary to account for the expected rewards over different periods of time in an instance charecterization, as opposed to the isolated instantaneous gaps, $(\Delta_t)_t$. 
%% thus rendering the instantaneous gaps insufficient.
%Towards overcoming this drawback,
%we introduce a derived structure 
%that we call \emph{detectable gap} profile that at every time-step 
%captures/accommodates/assimilates the details of a local gap profile taken over a local window of time.
% The window of time over which a detectable gap is the is suitably chosen based on the 
% detectable gap itself.
Precisely,
we define % the detectable gap profile, $\lambda = (\lambda)_t$, where for all $t \in [T]$,
\begin{align*}
    \lambda_t = 
    % \left\{
    \begin{dcases}
    	\max \left\{ \lambda \in [0,1] : \frac{1}{w(\lambda)}\abs{\sum_{t'=s}^t \mu_{1,t'} - \mu_{2,t'}} \geq \lambda  \right\}
        \quad &\text{, if such a $\lambda \in [0,1]$ exists.} \\ 
    	\sqrt{\frac{c_0 \log T}{t}} \quad &\text{, otherwise.}
    \end{dcases}
    \numberthis \label{eqn:lamdba-curve}
    % \end{array}
     % \right\}
\end{align*}

Here, $s:=t-w(\lambda)+1$ stands for the starting time-step of a sampling window
of size $w(\lambda) := \ceil{\frac{c_0 \log T}{\lambda^2}}$ that terminates at $t$, and $c_0 = 144$ is a constant \footnote{In fact, in the remainder of the paper, all notations of the form $c_i$ shall be suitable universal constants.}. Intuitively, $\lambda_t = \lambda$ for some time-step $t$ implies that a gap of $\lambda$ can be detected with high probability by observing samples from both arms in the past $\approx \nicefrac{1}{\lambda^2}$ time-steps.
% $k=2$ is the number of arms.
Fig. \ref{fig:lambda-description} depicts the detectable gap profile and gap profile for a two-armed bandit instance. 

We shall see that the detectable gap profile better reflects the nature of a non-stationary problem instance. 
Specifically, for our algorithm, we shall obtain a regret upper bound (to be shown in Theorem \ref{thm:inst-dep-reg}) 
as a function of the detectable gap profile, $\lambda$, which is an instance-dependent quantity.




==> arXiv version/related-work.tex <==
\subsection{Related Work}
\label{subsec:related-work}

Non-stationarity in bandit optimization has been extensively studied and dates back to the seminal work of \cite{whittle1988restless} on restless bandits, in which arms' states (and thus their reward distributions) change according to Markovian dynamics (also see \cite{slivkins2008adapting}). The past few decades, however, have witnessed the growth of hybrid adversarial and stochastic bandit models for non-stationarity, where the distributions of arms across time can be set by an adversary ahead of time in an arbitrary manner. Among the many  examples of such models are the following; the abruptly changing (or switching) bandits setting \citep{garivier2011upper, auer2019adaptively}, where the distributions are piecewise stationary and can arbitrarily change at unknown time steps,
and then, the the total variation-budgeted setting or the drifting bandits setting introduced by \cite{besbes2014stochastic, besbes2019optimal}. The authors show that with a constraint on the total amount of successive changes in arms' reward means, it is possible to devise algorithms with guarantees on the dynamic regret that depend on the variation budget $V_T$ and total time horizon $T$ of order roughly $O(V_T^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}})$ (ignoring logarithmic factors).

In this drifting bandits regime, there have subsequently been multiple works 
that have focused on dropping assumption of knowledge of drift parameter \citep{karnin2016multi},
extension of that to contextual bandits \citep{luo2018efficient},
and achieving optimal minimax bounds therein \citep{chen2019new},
however, an instance-dependent regret bound characterization has so far remained elusive under any sort of drifting reward constraint.
Our results not only match these optimal regret rates in a minimax sense, but we also give a more instance-dependent regret characterisation for our algorithm in a slowly-varying drifting bandits setting. 
% and provide the first minimax regret lower bound for this setting that turns out to match that of the more general total variation-budgeted setting of Besbes et al. 

In terms of lower bounds, \cite{besbes2014stochastic} provide a lower bound of $\Omega\left(V_T^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} \right)$ that matched their algorithm's upper bound (upto logarithmic factors), 
thereby closing the door on any possible improvements to them in recent years.
However, we show a matching minimax lower bound for slowly-varying bandits with equivalent per-round drift limit, which is a stronger result as it applies to a more restricted class of problems instances.
 % we establish that slowly varying bandits are at least as hard as the general total variation-budgeted setting.

Perhaps the only other work that studies the exact slowly-varying non-stationary bandit setting that we consider here is that of \cite{wei2018abruptly}. They modify the sliding-window-UCB algorithm of \cite{garivier2011upper} to employ windows that grow in size with time to get the SW-UCB\# algorithm. 

% develop a sliding-window version of the classic upper confidence bound (UCB) bandit algorithm, 
% and show that its dynamic regret is, in the worst-case over slowly varying instances, at most  $O\left(T^{1-\frac{\alpha}{3}} \log T\right)$, where $\alpha$ is a function of the drift rate of the arms' rewards. Our results not only improve over this regret rate in a minimax sense, but we also give a more instance-dependent regret characterisation for our algorithm and provide the first minimax regret lower bound for this setting that turns out to match that of the more general total variation-budgeted setting of Besbes et al. 

==> arXiv version/sketch-instance-bound.tex <==
%\subsection{Instance-dependent regret bound}
% {\bf Proof sketch for Theorem \ref{thm:inst-dep-reg} (Instance-dependent regret bound).} 
\paragraph{Proof sketch for Theorem \ref{thm:inst-dep-reg} (Instance-dependent regret bound)} 
We establish useful properties about
the nature of the active and passive phases, the sizes of episodes,
the connection between the regret and the detectable gap, $\lambda$.

We first restrict our attention to a \emph{good} event, $\GoodEvent$, where all empirical means fall close to the reward means, 
which occurs with high probability. 
%Then, we do the rest of the analysis and bound the regret under the assumption of occurrence of $\GoodEvent$,
%and finally obtain the theorem via a conditional expectation as is common in the literature.

Then (Lemma \ref{lem:inactive-not-optimal} in the appendix), we show that
in every episode, a snoozed arm (if it exists) remains sub-optimal for the entirety of the passive phase.
Towards this, we show that,
for an episode $i$, when the statistical test passes, at some point of time (say $t'$) in the active phase,
we have the true reward means of the arms well separated, i.e., $\mu_{a,t'} - \mu_{b,t'} \geq f$ for some gap $f$.
Then, we argue that the snooze period is carefully chosen based on this guaranteed true gap $f$,
the drift limit $\delta$, and the active phase duration $\tau_i$ such that arm $b$ remains sub-optimal in it. With this, we note that only an optimal arm is played in the passive phase, and thus, 
our algorithm incurs regret only during the active phase, which we try to bound next.

Next, we upper bound the regret $R_i$ in episode $i$ based on $\tau_i$, the duration of the active phase.
We use the fact that the statistical test did not pass at time $g_i - 1 = t_i + \tau_i - 1$,
specifically the fact that no arm was $\lambTil$-better than the other. 
We deduce that, their empirical means, and by the good event assumption, also their true means (over a period of time) were not well separatable after alternately playing arms for $\tau-1$ time steps.
Put simply, for these $\tau-1$ time-steps, the gap between the arms was less. 
This helps us get the following bound for $R_i$, the regret in episode $i$ as a function of the active phase duration $\tau_i$: % $R_i \leq  1 + 6 \sqrt{(\tau_i-1) \log T}$.
%
\begin{align*}
        R_i &\leq  1 + 6 \sqrt{(\tau_i-1) \log T}. \numberthis \label{sketch:eqn-1}
\end{align*}

This expression is also used (as a starting step) in the minimax regret upper bound derivation.
However, here, we go on to make a connection between $\tau_i-1$ and the detectable gap profile, $\lambda$.

Based on the design of detectable gap, we show, in Lemma \ref{lem:gauge-lambda-curve-relation}, that, if, for some $\tau >0$, at time $t'=t_i + \tau$ we have
$\lambda_{t'} > \sqrt{\frac{c_2 \log T}{\tau}}$, then our algorithm will surely (under occurrence of $\GoodEvent$) detects
a gap sufficient to declare $a >_{\lambTil} b$, and the statistical test shall pass. However, given that the statistical test did not pass at $g_i - 1 = t_i + \tau_i - 1$, 
we derive the instance-dependent episodic regret bound $R_i \leq c_4. \frac{1}{\lambda_{g_i - 1}} \log T + c_5$.

%\begin{align*}
%    R_i \leq c_4. \dfrac{1}{\lambda_{g_i - 1}} \log T + c_5 \numberthis \label{sketch:eqn-2}
%\end{align*}

We next collect all the episodic regrets to obtain the total regret,
For this, we analyze the episode durations in two possible cases:
episodes with a passive phase, and episodes without a passive phase, and show (Lemma \ref{lem:size-of-episode}) that in both cases, 
the minimum duration of any episode is $x = c_3 \delta^{\nicefrac{-2}{3}} \log ^{\nicefrac{1}{3}} T$. We also partition the time horizon $[T]$ into blocks of size $x$, and argue that each block can intersect with at most two episodes
as no episode can be fully contained within a block.

Finally, we account the regret of an episode to a block it intersects with, 
and aggregate over blocks the instance dependent regrets of episodes, via the per-episode regret bound %(by a further application of eqn. \ref{sketch:eqn-2})
to arrive at the final instance-dependent regret bound.



==> arXiv version/sketch-lower-bound.tex <==
%\subsection{Lower Bound}
%\label{sub-sec:lower-bound}

\paragraph{Proof sketch for Theorem \ref{thm:lower-bound} (Worst-case regret lower bound)}

We derive this result with information-theoretic arguments commonly employed in bandit literature \cite{garivier2016optimal}.

First, we adapt the standard change of measure inequality for sequential sampling (see e.g., \cite{garivier2019explore}) to a version that can accommodate non-stationary reward distributions.
Second, we break the time horizon into suitably small blocks of size $m$, establish lower bounds within each of them, 
and finally aggregate them to arrive at the lower bound expression.
Towards proving the lower bound within a block, we consider a base instance $\nu$, where both arms are identical and stationary with $\bern{\nicefrac{1}{2}}$ reward distributions.
We design a confusing instance, $\nu'$, where one arm is stationary with $\bern{\nicefrac{1}{2}}$ rewards, whereas,
the other arm (say, arm $1$, with a distribution of $\nu'_{1,t}$ at time $t$ within the block) exhibits non-stationarity as follows: $ \nu'_{1,t}$ is a Bernoulli distribution with parameter $\frac{1}{2} + \frac{t-1}{m} \varepsilon$ if $t \leq \ceil{\frac{m}{2}}$, and $\frac{1}{2} + \frac{m-t}{m} \varepsilon$ otherwise.

%	\begin{equation*}
%	    \nu'_{1,t} =
%	    \begin{dcases}
%	        \bern{\dfrac{1}{2} + \dfrac{t-1}{m}.\varepsilon} \quad & \text{if  } t \leq \ceil{\dfrac{m}{2}}\\
%	        \bern{\dfrac{1}{2} + \dfrac{m-t}{m}.\varepsilon} \quad & \text{if  } t > \ceil{\dfrac{m}{2}}\\
%	    \end{dcases} 
%	\end{equation*}

Essentially, within a block, arm $1$ starts identical to arm $2$ (with $\bern{\nicefrac{1}{2}}$ rewards), and for the first half of the block, drifts (by a suitably chosen value $\varepsilon$) upwards and away from a mean of $\nicefrac{1}{2}$, and reaches a maximum reward mean gap at half-way point.
Then, for the remainder of the block, it drifts towards (downwards) a mean of $\nicefrac{1}{2}$ and reaches back the $\bern{\nicefrac{1}{2}}$ reward distribution at the end of the block.

With this setup, we argue that when presented with a randomly chosen bandit problem instance
between $\nu$ and $\nu'$, any algorithm is condemned to incur in expectation the stated minimum regret.







==> arXiv version/sketch-minimax-upper.tex <==

%\subsection{Minimax regret bound}

\paragraph{\bf Proof sketch of Theorem \ref{thm:minimax-bound} (Minimax regret bound)} 

For every episode $i$, we upper bound the \emph{average regret} or per time-step regret defined as $R^{ave}_i = O\left(\frac{R_i}{ t_{i+1}-t_i}\right)$.
Then, we shall argue that the regret is bounded by $T$ times the maximum average regret incurred by any episode.

From eqn. \ref{sketch:eqn-1}, we have the regret in an episode $i$ dependent on the active phase duration $\tau_i$ 
as $R_i = O\left( \sqrt{\tau_i \log T} \right)$.

We analyse $R^{ave}_i$ based on the following two cases based on the presence or absence of a passive phase.

\paragraph{Case $\tau_i < \text{buf}$ :}  
Equivalently, we have $\tau_i < \frac{2}{\delta} \sqrt{\frac{\log T}{\tau_i}}$, and thus $\tau_i < 2^{\nicefrac{2}{3}} \delta^{\nicefrac{-2}{3}} \log^{\nicefrac{1}{3}} T$.
As this episode has a passive phase, the duration of this episode, $t_{i+1} - t_i = \text{buf} = \frac{2}{\delta} \sqrt{\frac{\log T}{\tau_i}}$. 
With these, the average regret is bounded as $R^{ave}_i = O\left(\dfrac{\sqrt{\tau_i \log T}}{\frac{1}{\delta}\sqrt{\frac{\log T}{\tau_i}}}\right) = O\left(\tau_i \delta\right) = O\left( \delta^{\nicefrac{1}{3}} \log^{\nicefrac{1}{3}} T \right)$.

\paragraph{Case $\tau_i \geq \text{buf}$ :} Equivalently, $\tau_i \geq \frac{2}{\delta} \sqrt{\frac{\log T}{\tau_i}}$ and thus,
$\tau_i \geq 2^{\nicefrac{2}{3}} \delta^{\nicefrac{-2}{3}} \log^{\nicefrac{1}{3}} T$.
Here, the episode $i$ does not have a passive phase. Thus, the duration of this episode is $t_{i+1} - t_i = \tau_i$.
With these, the average regret is bounded as 
$ R^{ave}_i = O \left( \frac{ \sqrt{\tau_i \log T} }{\tau_i} \right) 
= O\left(\sqrt{\frac{\log T}{\tau_i}} \right) 
= O\left(\delta^{\nicefrac{1}{3}} \log^{\nicefrac{1}{3}} T \right) $.

From both cases, as the maximum per-time step regret is similarly bounded,
we multiply this by the length of the horizon, $T$, to show the desired minimax bound of $O\left(T \delta^{\nicefrac{1}{3}} \log^{\nicefrac{1}{3}} T\right)$.


Optionally, we refer the reader to appendix \ref{appn-sub-sec:ave-reg-by-epis-variables} for 
an assessment of the interplay between average regret in an episode, its total duration, and its active phase duration.

% \begin{corollary}
%     For a slowly varying bandit problem with a drift limit $\delta = T^{-\kappa}$,
%     $\AlgGE$ incurs an expected regret of  
%     $O \left(T^{1-\nicefrac{\kappa}{3}} \log^{\nicefrac{1}{3}} T \right)$.
% \end{corollary}



==> arXiv version/sketches.tex <==
\section{PROOF SKETCHES}

The formal proofs of all results are deferred to the appendix (\ref{appn-sec:instance-upper-bound}, \ref{appn-sec:minimax-upper}, and \ref{appn-sec:low-bound}) in the interest of space. 

%In the interest of space, we defer the formal proofs of the Theorems to Appendix \ref{appn-sec:instance-upper-bound}, \ref{appn-sec:minimax-upper}, and \ref{appn-sec:low-bound}.
%In this section (the following sub-sections), we give proof-sketches for the Theorems. 
% and give key idea
% and discuss our results in contrast with the literature.

\input{sketch-instance-bound}

\input{sketch-minimax-upper}

\input{sketch-lower-bound}



==> arXiv version/theoretical-guarantees.tex <==

\section{THEORETICAL GUARANTEES}
\label{sec:guarantees}

Our first main result is a regret bound for the $\AlgGE$ algorithm in terms of the detectable gap profile of a slowly-varying bandit instance. 

\begin{restatable}{theorem}{TheoremInstanceDependentUpperBound}[Instance-dependent regret bound]
\label{thm:inst-dep-reg}
    If $\AlgGE$ is run with a drift limit parameter $\delta$ on a problem instance $\mu \in S_\delta$,
    % Given a problem instance $\left(\mu=\left(\mu_{1,t}, \mu_{2,t} \right)_{t=1}^{T}, \delta \right)$,
    then its expected regret satisfies
    \begin{align*}
         R(\AlgGE) \leq c_8 + c_6 \sum_{j=1}^{m} \frac{1}{\lambda_{min}(j)}. \log T + c_7,
    \end{align*}
    where $m = \nicefrac{T}{\tau}$ is the number of blocks, 
    each of length not more than $\tau = \min\left\{T, c_3 \delta^{\nicefrac{-2}{3}} \log^{\nicefrac{1}{3}} T\right\}$,
    and for every block $j \in [m]$ spanning a time period $b_j := [(j-1)\tau + 1, j\tau] \cap [T]$, 
    $\lambda_{min}(j) := \min_{t \in b_j}\lambda_t$.
    Here, $c_i$s are suitable constants.
\end{restatable}

We also have the following upper bound on the worst-case (over instances in $S_\delta$) regret for \AlgGE.

\begin{restatable}{theorem}{TheoremMinimaxUpperBound}[Minimax Upper bound]
\label{thm:minimax-bound}
    If $\AlgGE$ is run with a drift limit parameter $\delta$ on a problem instance $\mu \in S_\delta$, $\AlgGE$ incurs an expected regret of
    $O\left(T \delta^{\nicefrac{1}{3}} \log^{\nicefrac{1}{3}} T \right)$.
\end{restatable}

We finally complement the worst-case regret upper bound for $\AlgGE$ with a matching universal minimax regret lower bound: 

\begin{restatable}{theorem}{TheoremLowerBound}[Minimax Lower Bound]
\label{thm:lower-bound}
For any algorithm $\Alg$ and a drift limit $\delta > 0$, there exists a problem instance $\mu \in S_\delta$ such that,
$\Alg$ incurs a expected regret of
$\Omega\left(T \delta^{\nicefrac{1}{3}}\right)$.
\end{restatable}

%We have the following corollary for $\delta = T^{-\kappa}$:

% \begin{corollary}
% 	\label{cor:low-bound-kappa}
% 	For the slowly-varying bandit problem with a drift limit $\delta = T^{- \kappa}$, 
% 	the worst-case expected regret for any algorithm $\Alg$ is
% 	$\Omega\left(T^{1-\nicefrac{\kappa}{3}}\right)$.
% \end{corollary}

\paragraph{Discussion} The minimax regret lower bound we obtain establishes (constructively) that if the drift limit $\delta = \Omega(1)$, then it is impossible to achieve a sub-linear (in time) regret for any algorithm.
The interesting problem space is thus when $\delta = o(1)$\footnote{as a function of total time $T$}.
% $S_{o(1)}$, that

A basic sanity check is to evaluate our results for the stationary bandits setting, that is when $\delta = 0$, and the gap $\Delta$ is unchanged over time.
In that case, in Theorem \ref{thm:inst-dep-reg}, the size of a block is $\tau=T$.
From the detectable gap definition, either with $\lambda_t = \Delta$ from the first assignment, or $\lambda_t > \Delta$ from the second,
we have $\lambda_t \geq \Delta$ at all times $t$.
This gives us a regret bound of $O\left( \frac{1}{\Delta} \log T\right)$. One can also observe that $\AlgGE$ behaves similar to the classical Successive Elimination algorithm in this regime.
After it distinguishes the optimal arm from the sub-optimal, that is, the statistical test passes,
it computes a sub-optimality buffer $\text{buf}=\frac{2}{\delta} \sqrt{\frac{\log T}{\tau_i}} = \infty$, an infinite passive phase,
i.e., it snoozes the sub-optimal arm indefinitely.

Moving on, for non-stationary instances with small positive drift limits -- specifically, 
for $\delta \leq O\left(\frac{\log^{\nicefrac{1}{2}}T}{T^{\nicefrac{3}{2}}} \right)$ -- applying 
Theorem $\ref{thm:inst-dep-reg}$ still yields a block size of $\tau=T$. With a similar analysis, this results in a regret bound of $O\left( \frac{1}{\Delta} \log T\right)$\footnote{With the drift, consider the smallest value of $\Delta_t$ for the expression, or corresponding $\lambda_t$ value.}. 
For $\Delta = \Theta(1)$, it is noteworthy that our results show a logarithmic regret despite the mild non-stationarity of the instance, which, to the best of our knowledge, has not been shown before.
% is a first-of-its-kind result.

This result in Theorem \ref{thm:minimax-bound} is comparable with that of \cite{besbes2014stochastic} who work on a total variation-budgeted setting.
In our setting, a drift limit of $\delta$ per time-step translates to a cumulative drift limit of $T \delta$ over the entire time horizon.
Precisely, for an arm $a$,
$\sum_{t=1}^{T-1} \abs{\mu_{a,t} - \mu_{a,t+1}} \leq T \delta$.
This cumulative drift limit quantity is termed the variation budget $V_T$ in theirs,
and we, here, have $V_T = T \delta$.
Substituting this in their regret upper bound $O\left(T^{\nicefrac{2}{3}} V_T^{\nicefrac{1}{3}} \log ^{\nicefrac{1}{3}} T\right)$,
we get $O\left(T \delta^{\nicefrac{1}{3}} \log^{\nicefrac{1}{3}} T \right)$, the same upper bound as ours.
Thus, we note that our minimax upper bound matches that of \cite{besbes2014stochastic} which accomodates a more general setting.
On a more intereting note,
substituting $V_T = T \delta$ in their regret lower bound $\Omega(T^{\nicefrac{2}{3}} V_T^{\nicefrac{1}{3}})$,
we get $\Omega\left(T \delta^{\nicefrac{1}{3}} \right)$, the same lower bound expression that we have established.
Thus, we note that our minimax lower bound matches that of \cite{besbes2014stochastic},
and crucially establishes that the seemingly easier slowly-varying bandits problem 
is at least as hard as the more general budgeted drifting bandit problem in a minimax sense.

